TABOR: A Highly Accurate Approach to Inspecting and Restoring Trojan Backdoors in AI Systems

A trojan backdoor is a hidden pattern typically implanted in a deep neural network. It could be activated and thus forces that infected model behaving abnormally only when an input data sample with a particular trigger present is fed to that model. As such, given a deep neural network model and clean input samples, it is very challenging to inspect and determine the existence of a trojan backdoor. Recently, researchers design and develop several pioneering solutions to address this acute problem. They demonstrate the proposed techniques have a great potential in trojan detection. However, we show that none of these existing techniques completely address the problem. On the one hand, they mostly work under an unrealistic assumption (e.g. assuming availability of the contaminated training database). On the other hand, the proposed techniques cannot accurately detect the existence of trojan backdoors, nor restore high-fidelity trojan backdoor images, especially when the triggers pertaining to the trojan vary in size, shape and position. In this work, we propose TABOR, a new trojan detection technique. Conceptually, it formalizes a trojan detection task as a non-convex optimization problem, and the detection of a trojan backdoor as the task of resolving the optimization through an objective function. Different from the existing technique also modeling trojan detection as an optimization problem, TABOR designs a new objective function--under the guidance of explainable AI techniques as well as heuristics--that could guide optimization to identify a trojan backdoor in a more effective fashion. In addition, TABOR defines a new metric to measure the quality of a trojan backdoor identified. Using an anomaly detection method, we show the new metric could better facilitate TABOR to identify intentionally injected triggers in an infected model and filter out false alarms......

==> eval.tex <==
\section{Evaluation}
\label{sec:3}

\textcolor{red}{This section is ready for reviewing and modifying except the follwing problems. The problems need to be solved by experiments and the experiments are being run step by step.}

\textcolor{red}{todo: 
1. example: why some examples are bad in Table 2. compute a ratio to explain. add average.
2. visualize the trojan better. 
3. Table 7 empty model.
4. comparison experiments for model complexity, advanced trojan? Robustness in Hyper-Parameter explanation. Add explanation why we choose those hyper-parameter values.
6. patch the trojan and show the second one.
7. move the metric to tech.
9. model atchitecture: appendix or here. wait to see.
11. show the false positive.
12. 100\% accurate results in top left square gtsrb. add explanation? how to design the metric? top left back ground noise.
13. ask Wenbo for clean model. add false positive number to the table.
}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,fill,inner sep=0.5pt] (char) {\textcolor{white}{#1}};}}

In this section, we describe our implementation, the dataset we utilized, set up our experiments, and summarize our experimental results. Through this evaluation, we seek to answer the following questions. 
\circled{1} Compared with the state-of-the-art: Cleanse \cite{wang-2019-ieeesp}, does the proposed approach exhibit better performance in terms of fidelity of the detected trojan and robustness when the trojan varies in size, position, shape and attack method?
\circled{2} Can the proposed technique accurately detect trojan in high-dimension search space where Cleanse \cite{wang-2019-ieeesp} cannot?
\circled{3} Can the improvement in fidelity and robustness contribute to the accuracy of end-to-end trojan detection, and thus bring positive impact upon the capability in real-world trojan detection system?

\subsection{Experimental Setup}
\label{subsec:3.1}

\textbf{Datasets:} In order to answer the three questions mentioned above, we choose to evaluate our strategy on three datasets with different tasks, input sizes, number of classes and training samples: GTSRB \cite{GTSRB}, PubFig \cite{PubFig} and ImageNet \cite{imagenet_cvpr09}. 

GTSRB is a small dataset designed for traffic sign recognition. PubFig is a widely-used face recognition dataset. They are both evaluated in Cleanse paper \cite{wang-2019-ieeesp}, which allows a direct comparison with our strategy (to answer \circled{1}).

ImageNet is probably the most widely-used dataset in computer vision for object classification and recognition. We choose it to better demonstrate our approach's superiority on high-dimensional input images (to answer \circled{2}) together with PubFig. The details of used datasets are included in Table \ref{tab:datasets}.

\input{table/dataset.tex}

\noindent\textbf{Model Architecture: } In this paper, we focus on trojan injected in classification task. We choose the same classification model as in Cleanse paper \cite{wang-2019-ieeesp} for GTSRB and PubFig for direct comparison. We train VGG16 \cite{simonyan2014very} on ImageNet. The architectures of the models are shown in Table \ref{tab:models}.

\input{img/model.tex}

\noindent\textbf{Attacks:} In order to show that our strategy can detect trojan injected by different attacks, we apply two mainstream trojan attack methods  to our models: BadNet \cite{gu2017badnets} and Trojan Attack \cite{Trojannn}. More speicfically, we apply BadNet to inject trojan in models trained on GTSRB and ImageNet, and Trojan Attack to poison models trained on PubFig.

\subsection{Experimental Design}

Using the poisoned models as well as the datasets described in Section \ref{subsec:3.1}, we set up a series of experiments to evaluate our proposed technique and thus answer the three questions presented above. 

To answer the first question \circled{1}, we use both Cleanse and our technique to detect the trojans in poisoned models trained on GTSRB, PubFig and ImageNet. We then calculate fidelity metrics on the results to evaluate the fidelity of the detected trojan. In order to evaluate robustness of detection, we vary the trojan by size, shape, and position on GTSRB and ImageNet. To test robustness against different attack methods, we apply BadNet attack \cite{} on GTSRB and ImageNet and Trojan Attack \cite{} on PubFig. We also use different attacks to inject trojan as illustrated in Section \ref{subsec:3.1}. The results on high-dimensional datasets: ImageNet and PubFig, can also answer the second question \circled{2}.

To answer the last question \circled{3}, we set up an end-to-end experiment comparing our proposed method with Cleanse. In the end-to-end experiment, the first step is to detect trojans in all classes, because in real-world applications, prior knowledge of the target class is unavailable. The second step is to apply an anomaly detection method to all the results. The intuition is that if a trojan is injected in the class, the detecting result will be pretty different from those classes which is not poisoned. If there is any anomaly result detected, the system will report a trojan detected with the corresponding target label. We compare our approach with Cleanse in terms of detection success rate and accuracy of the detected target label.

\noindent\textbf{Fidelity Metrics: } In order to evaluate the fidelity of the detected trojan compared with the original trojan, we introduce five numerical metrics reflecting different aspects of the similarity between the detected trojan and original trojan.

\begin{itemize}
    \item Mask $l_1$ Distance: We take the $l_1$ distance between masks as a metric for \emph{shape} similarity between the detected trojan and the original trojan.
    \begin{equation}
        d_{m, l_1} = ||m_d-m_{trojan}||_1
    \label{eq:mask_l1}
    \end{equation}
    \item Delta $l_2$ Distance: We take the $l_2$ distance between patterns as a metric for \emph{shape} and \emph{color} similarity between the detected trojan and the original trojan.
    \begin{equation}
        d_{\Delta, l_2} = ||\Delta_d-\Delta_{trojan}||_2
    \label{eq:delta_l2}
    \end{equation}
    \item Precision: The area of the overlapping part of the detected trojan and the original trojan divided by the area of the detected trojan. Precision can be seen as a measure of exactness or quality of the detected trojan.
    \begin{equation}
        precision = \frac{||m_d*m_{trojan}||_1}{||m_d||_1}
    \label{eq:precision}
    \end{equation}
    \item Recall: The area of the overlapping part of the detected trojan and the original trojan divided by the area of the original trojan. Recall is a measure of completeness of the detected trojan. Note that when the trojan is large, we usually only detect the border of the trojan which will result in a low recall score but does not mean the detection result is bad.
    \begin{equation}
        recall = \frac{||m_d*m_{trojan}||_1}{||m_{trojan}||_1}
    \label{eq:precision}
    \end{equation}
    \item The harmonic average of precision and recall. Reflects the average performance considering precision and recall.
    \begin{equation}
        F_1 = \frac{2*precision*recall}{precision+recall}
    \label{eq:f1}
    \end{equation}
\label{item:fidelity_metric}
\end{itemize}


\textcolor{blue}{todo for Wenbo: move this to the techinque part.}
\noindent\textbf{End-to-end Detection Metrics: } We use \emph{magnetic anomaly detection (MAD)} to pick out the real trojan in an end-to-end detection. MAD requires a metric for the anomaly detection in the end-to-end detection. In Cleanse \cite{wang-2019-ieeesp}, they simply use the $l_1$ norm of the detected mask. However, this is not good in that a small area is not the only thing that gives confidence to a detected trojan. Thus we propose a new metric as following.

\begin{equation}
    \textcolor{blue}{todo for Wenbo: add new metric}
\end{equation}

\textcolor{blue}{todo for Wenbo: add explanation for new metric}

\subsection{Experimental Results}

\input{table/fidelity.tex}

\noindent\textbf{GTSRB: } In order to evaluate the robustness of our proposed method, we vary the shape, size, position of the trojan injected in models trained on GTSRB. Specifically, we inject white square on top left and bottom right, and firefox on top right and bottom left. With each combination of the shape and position, we vary the size of the injected trojan in [6*6, 8*8, 10*10, 12*12, 14*14]. We evaluate both our approach and Cleanse in the same settings for a direct comparison.

The fidelity results are shown in Figure \ref{tab:fidelity}. Note that the better result between our technique and Cleanse is bolded in \ref{tab:fidelity}. We can see that our approach beats Cleanse in every setting with both $l_1$ and $l_2$ distances on GTSRB. The improvement can also be double-confirmed by the visual results in \ref{tab:res_gtsrb}. This means that our detected trojan is more similar to the original trojan in terms of shape and color. We can also tell from table \ref{tab:fidelity} that our approach is always better in terms of precision but sometimes not as good in recall. This is because Cleanse sometimes detect a much larger area than the original trojan leading to a high recall score but does not necessarily mean a better detection result. This means that our detected trojan is more compact and precise while Cleanse tend to give a large and rough result. 

The performance improvement owes to the new loss terms in our technique. Specifically, by adding the new loss terms, we better guide the optimization process via sharking the searching space of the trojan, filtering out false positive and enhancing trojan fidelity as described in Section \ref{sec:tech}. These augmentations help us (1) avoid adversarial examples like the one detected on top right in ImageNet with Cleanse when actually a 80*80 firefox trojan is injected on top right. (2) fine-tune the detected trojan to get rid of the redundant part and give a more compact and precise result. 

\input{table/res_gtsrb.tex}

% \input{table/fidelity_gtsrb.tex}

\noindent\textbf{ImageNet: }
In order to evaluate the robustness of our proposed method, we vary the shape, size, position of the trojan injected in models trained on ImageNet. Specifically, we inject white square on top left and bottom right, and firefox on top right and bottom left. With each combination of the shape and position, we vary the size of the injected trojan in [20*20, 40*40, 60*60, 80*80, 100*100]. We evaluate both our approach and Cleanse in the same settings for a direct comparison.

The fidelity results are shown in Figure \ref{tab:fidelity}. Note that the better result between our technique and Cleanse is bolded in \ref{tab:fidelity}. We can see that our approach beats Cleanse in most settings (with only 1 exception in Mask $l_1$ Distance and 4 exceptions in Delta $l_2$ Distance). \textcolor{red}{The difference in fidelity score is close in some settings which does not fully reflect the improvement because when trojan size is large, the detected trojan is usually the border of the injected trojan, but Mask $l_1$ Distance and Delta $l_2$ Distance cover the whole trojan area, which will dilute the impact of accurate detection of the border.} This can be confirmed by the precision, recall and $F_1$ score. We can see that in most settings, the precision, recall and $F_1$ score of our approach are much better than those of Cleanse. \textcolor{red}{There is only one
conspicuous exception where our approach are defeated in every metric when a 20*20 firefox trojan is injected on bottom left in ImageNet. Because there is only one of it, we take it as a rare random result.}  The general improvement can be more accurately reflected in the visual results in \ref{tab:res_gtsrb}. We can see that trojans detected by our approach are more similar to the injected trojans' border in most cases. In some firefox examples, you can even see the vortex inside firefox in the detected trojan (Bottom Left 40*40).

The improvement of detection on ImageNet can also be explained by the same reasons as in GTSRB. But we want to highlight that of all the reasons mentioned, filtering out false positive is the most important one for high-dimensional dataset like ImageNet. As we can see in Table \ref{tab:res_imagenet}, with Cleanse, there are many wrongly detected ``trojans'' (actually adversarial example) which even does not share the same location as the original trojan. By adding new loss terms, we successfully filter out these false positives and always manage to find the right trojan with a high fidelity.

\input{table/res_imagenet.tex}

\noindent\textbf{PubFig: }
In order to evaluate the robustness of our approach facing different attack methods, we attack PubFig using Trojan Attack \cite{liu2017trojaning}. The trojan and the detected result is shown in Figure \ref{tab:res_pubfig}. Our detected trojan is more close to the original one in position and shape, which means our approach has the ability to accomodate different kinds of trojan attacks.

\input{table/res_pubfig.tex}

\noindent\textbf{End-to-end Detection: }
Question \circled{3} is actually the most important one when we try to apply our detection technique in practice. \textcolor{red}{No matter how similar the detected trojan is to the injected trojan, if it cannot be picked out in an fully automatic end-to-end detection system, it is useless in real-world system.}

As shown in Table \ref{tab:end2end}, our approach can always successfully detect the injected trojan while Cleanse cannot in most cases especially high-dim ones. In order to better understand the results, we go through all the detection results. An interesting phenomena we observed is that when the input size grows, Cleanse tends to report adversarial example that is close to an injected trojan as shown in Figure \ref{} because when the dimension of the search space of the trojan becomes high, it is easier to find a trojan-like adversarial example to fulfill the \textcolor{red}{area restriction loss} in Cleanse.
Our approach, however, eliminate these trojan-like adversarial examples by adding the explanablity loss and smoothness loss. As a result, the trojans detected in the non-target labels are all as Figure \ref{tab:adv} which is so different from the trojans detected in the target label so anomaly detection can easily pick them out.
\textcolor{red}{todo: add the explanation for clean models after Wenbo gets the results.}

\input{table/end2end.tex}

\input{table/adv.tex}

\subsection{Miscellaneous Experiments}

Prior sections described and evaluated detection of trojans in order to answer the three most vital questions mentioned at the start of Section \ref{sec:3}. Besides the three questions, there are many other important but unsolved questions: Is our approach robust to hyper-parameter change? How will our technique perform when detecting advanced trojans like multiple trojans injected in one class? Will model complexity influence the detection result of our method? In this section, we set up some small-scale experiments and give both empirical results and probable theoretic explanation to these questions.

\noindent\textbf{Sensitivity of the hyper-parameters}
To test the robustness of our approach against hyper-parameters, we use 16 different combinations of hyper-parameters to detect 8*8 square trojan injected in bottom right GTSRB.
\textcolor{red}{Specifically, we vary $\lambda_4$ between $e^{-2}$ and $e^{-3}$, $\lambda_5$ between $e^{-4}$ and $e^{-5}$, $\lambda_6$ between $e^{-5}$ and $e^{-6}$, $\lambda_7$ between $e^{-6}$ and $e^{-7}$, and take the combinations of all of them. We choose to vary between these specific values balance the different loss terms. On GTSRB, when we choose the above hyper-parameters, the range of different loss terms are almost the same, guaranteeing that each term can take its effect as designed. Because the rough range of the loss terms can be known before running experiments, we claim it as a a guideline to set the initial hyper-paramenter values.}
The results are included in Table \ref{tab:hyper} and we can see that although the fidelity of the results are different, our approach successfully detect the rough position and shape of the trojan in all 16 settings. As a conclusion, we announce that our approach is relatively robust to hyper-parameter setting when the initial hyper-parameters are set to balance the different loss terms. This is a huge advantage in practice because it can mitigate the painful problem of hyper-parameter tuning.

\textcolor{red}{todo: add explanation for Cleanse after getting the results. the experiment has relatively low priority and is not being run now. Remember to start after other experiments.}

\input{table/hyper.tex}

\noindent\textbf{Advanced Trojan:} We have been considering normal trojan, that is injecting one trojan in one model with one target label, in the whole paper. However, we may encounter more complicate trojan than normal trojan. Multiple trojans injected in one model is the most common one.

\emph{Multiple Trojans in Single Label: }
Let's first consider the situation where multiple trojans are injected in one model with the same target label. We inject firefox in the bottom left and square in the bottom right in GTSRB with target label 33, and ImageNet with target label 0. The detection results are shown in Table \ref{tab:2_trojan_1_label}. We can tell that at least one trojan can always be detected using our approach. After patching the first detected trojan, the second one can be detected afterwards.

\textcolor{red}{todo: add results and explanation for patching after getting the results. the experiment is being run now.}

\input{table/2_trojan_1_label.tex}
An even more complicated situation is that multiple trojans are injected in the same model with different target labels. In order to figure out if our approach has the ability to detect all the trojans, we inject 2 trojans in 2 different labels with 4 different settings: bottom left firefox targeting at 0 and bottom right square targetting at 33 in GTSRB, and bottom left firefox targeting at 1 and bottom right square targeting at 0. And the results show that although this seems more tricky than the first situation, it is actually simpler for our approach to deal with. We can just detect the trojans in all labels as we always do and report the anomaly ones. As shown in Table \ref{tab:2_trojan_2_label}, our approach can correctly detect 2 trojans injected in 2 different labels on both GTSRB and firefox.

The above two sets of experiments show that our approach has the basic ability to detect advanced trojans.

\input{table/2_trojan_2_label.tex}

\noindent\textbf{Influence of Model Complexity: }
It is also unclear how model complexity will affect the performance of our approach. Intuitively, the more complex the model is, the harder it is to find a hidden trojan in it. This intuition is partially sealed by results in Table \ref{tab:complexity}. We train a shallow network and a deep network on both GTSRB and ImageNet. The detection results are similar, but the fidelity is better with shallow networks. A possible explanation is that the more complex the model architecture is, the more \textcolor{red}{twisty (not sure if this is the correct word for here)} the manifold is. The distance between edge examples and the manifold is thus smaller and bypassing is easier. This indicates the expansion of the adversarial example space, and thus increase the difficulty finding the correct trojan.

\input{table/complexity.tex}

==> note.tex <==
\section{Key Technique}
\label{sec:tech}

% In this section, we first describe the design principle of a trojan backdoor detection approach. Then, we conduct an empirical study to analyze those trojan backdoors the state-of-the-art technique mistakenly identified. Following our analysis, we introduce the detail of our trojan detection technique.

% \subsection{Design Principle}
% \label{subsec:principle}

As is discussed in a pioneering research work~\cite{}, given an infected model, detecting an injected trigger can be viewed as solving the following optimization
%
\begin{equation}
\label{eq:1}
\begin{aligned}
    \text{argmin}_{\bd, \bM} L(f(\bx_t), y_{t}) \, , \\
    \bx_t = \bx \odot (\mathbf{1} - \bM) + \bd \odot \bM \, , 
\end{aligned}
\end{equation}
%
Here, $\bM$ and $\bd$ are a mask and a pattern, respectively. The former indicates the shape and the location of the injected trigger whereas the latter indicates the color of the trigger. When multiplied together (i.e., $\bM\odot\bd$), they denote the trigger restored (see Figure~\ref{fig:trojai01}). In the equation above, $\bx \in \mathbb{R}^{d \times d}$ is a testing sample in matrix form\footnote{Note that if an input is a colored image, $\bx$ should be a 3-D tensor of ${R}^{d \times d \times 3}$ instead of a 2-D matrix.} and $\bx_t$ denotes the data sample $\bx$ with the trigger $\bd \odot \bM$ inserted (see Figure~\ref{fig:trojai01}). $y_{t}$ represents a specific target class, into which the model $f(\cdot)$ misclassifies arbitrary contaminated inputs (\ie $\bx_t$). The loss function $L(f(\bx_t), y_{t})$ indicates the similarity between the prediction $f(\bx_t)$ and the target class $y_{t}$. 

If a trojan backdoor exists and could misclassify a trigger-inserted image into a target class $y_{t}$, ideally, one could obtain a solution for $\bd$ and $\bM$ from the optimization above, deem $\bd \odot \bM$ as the corresponding trigger backdoor and eventually conclude the model $f(\cdot)$ contains a trojan. Otherwise, she can conclude the model is clean, carrying no trojans. However, for any given value of $y_{t}$ and model $f(\cdot)$, it is not difficult to note that one can always obtain a solution (i.e., a local optimum) for $\bd$ and $\bM$ simply because of the non-convex property of DNNs~\cite{}. 

For a clean model $f(\cdot)$, the local optimum indicates a false alarm but not a trigger pertaining to an intentionally-inserted trojan backdoor. For an infected model $f(\cdot)$, the local optimum may represent the trigger intentionally inserted or an incorrect trigger (i.e., an unintentionally-inserted trigger tied to a non-target class or a trigger tied to the target class but with nearly no overlaps with the trigger intentionally inserted). 

As is mentioned in Section~\ref{subsec:scope}, the goals of a model user are to (1) point out whether a model truly carries a trojan backdoor intentionally implanted but not those naturally existing and (2) if an intentionally inserted trojan exists, restore the corresponding trigger. Therefore, in order to obtain the best trojan detection performance, a trojan detection technique has to minimize the negative influence of false alarms as well as incorrect triggers. In this work, we tackle this issue by (1) conducting an empirical study to analyze the false alarms as well as incorrect triggers and (2) designing a new objective function to eliminate unexpected local optima. 


% tied to could be an incorrect trigger or the one corresponding to that trojan. It should be noted that, by inserting a false alarm or an incorrect trigger into an image, a misclassification can be observed. However, as is mentioned in Section~\ref{}, the goals of a model user are to (1) point out whether a model truly carries a trojan intentionally implanted but not those naturally existing and (2) if an intentionally inserted trojan exists, restore the corresponding trigger. Therefore, an effective trojan detection approach should be able to not only eliminate false alarms but also correctly identify and restore the trigger truly tied to the trojan intentionally inserted. With the first capability, the trojan detection approach could help an end user accurately point out the existence or non-existence of a trojan backdoor. With the second capability, it could facilitate the model user's ability to take further actions (e.g., fixing the infected model by patching that trojan backdoor). It should be noted that, this work does not assess the effectiveness of a trojan detection approach by using its capability in minimizing incorrect triggers. This is because, as long as false alarms are removed and the actual triggers are accurately restored, even with the existence of incorrectly identified triggers, a model user can still correctly conclude whether a trojan is actually enclosed and even apply an effective patch to an infected model. 



As is mentioned above, for false alarms and incorrect triggers, one of their characteristics is their overly-large sizes. Therefore, when resolving the aforementioned optimization, we can introduce a regularization term to penalize the resolved triggers overly large. Technically speaking, this can be interpreted as restricting the size of the trigger resolved or in other words controlling the number of non-zero elements in $\bM$. With this penalization, when searching solutions in adversarial subspace, we can ensure the optimization could have better chance to converge at a local optimum indicating the trigger pertaining to the inserted trojan. Conceptually, this can be viewed as we shrink the adversarial subspace by removing all the adversarial samples carrying a overly-large trigger.  

Recall that we observe resolved triggers blocking the key object in images. To eliminate triggers in this category, we leverage the definition of trojan backdoors. As is mentioned in Section~\ref{subsec:scope}, in order to avoid blocking key objects in an input image, a malicious trigger is usually present at the corner of an input image. Therefore, by simply removing the trigger (or technically speaking nullifying the corresponding pixels) from a trigger-inserted image, a model should be able to correctly classify that trigger-removal image. In this work, we utilize this definition to derive a heuristic, and then design a regularization term by using this heuristic. 

In addition to the blocking triggers, recall that we also observe the triggers that overlay the trigger pertaining to the trojan intentionally inserted. As is discussed in Section~\ref{} (Observation III), while this kind of trigger is correctly tied to the trigger of our interest, it is not beneficial for 


Recall that we observed resolved triggers blocking the key object in images. To eliminate triggers in this category, we leverage the definition of trojan backdoors. As is mentioned in Section~\ref{subsec:scope}, in order to avoid blocking key objects in an input image, a malicious trigger is usually present at the corner of an input image. Therefore, by simply removing the trigger (or technically speaking nullifying the corresponding pixels) from a trigger-inserted image, a model should be able to correctly classify that trigger-removal image. In this work, we utilize this definition to derive a heuristic, and then design a regularization term by using this heuristic. We integrate this regularization into optimization and thus eliminate the images with blocking triggers from adversarial sample subspace. 

In addition to the blocking triggers, recall that we also observe triggers that overlay the trigger pertaining to the trojan intentionally inserted. As is discussed in Section~\ref{subsec:obs} (Observation III), while this kind of triggers is correctly tied to the trigger of our interest, they do not represent a high-fidelity restoration. To address this problem and improve fidelity for resolved triggers, we design a regularization term by borrowing the idea of those explainable AI techniques (e.g.,~\cite{}). The rationale behind our design is as follows. 

An overlaying trigger indicates a trigger with additional irrelevant features enclosed. When presenting an input with an overlaying trigger, even if we remove all the features except for the features tied to the trigger pertaining to the inserted trojan, an infected model should still output an incorrect result. Therefore, the most effective approach to restoring the trigger pertaining to an inserted trigger is to knock off all the features, preserve the minimal set of features and deem the remaining set as the trigger intentioned inserted. For explainable AI techniques, their goal is to identify the most important features contributing to a classification result. Given an input sample $\bx_{t}$ with a resolved trigger attached, an explainable AI technique therefore could assess the feature importance, eliminate those features not dominant to the misclassification and eventually provide us with a trigger in a higher fidelity.

==> outline.tex <==
    1. Introduction. (1.5)
    Problems of existing Trojan detection techniques.
        -- Cannot deal with high dimensional inputs (larger search space).
            -- Cannot correctly recovering the original Trojan shape (l1 norm dosenot performs well in high dimensional space). 
            -- Including false positive (dosenot filtering out adversarial samples).
            -- Cannot obtaining high fidelity Trojan (dosenot adding any constraints on delta). 
    Challenge：
        -- How to shrink the searching space.
        -- How to filter out the false positive.
        -- How to get a high fidelity Trojan. 
    Solution：
        -- How to shrink the searching space.
            -- Using other norm instead of l1 (nuclear and elastic-net).
        -- How to filter out the false positive.
            -- Adding smoothness loss.
        -- How to obtain a high fidelity Trojan. 
            -- Adding similar loss on delta.
            -- integrating the explanation part.

2. Background and Threat model (1 page)
    2.1 Backdoor
    2.2 Threat model and assumption (Existing attacks)

3. limitation and Problem Scope.
    3.1 Limitation of existing Trojan detection. (goes to 3)
        -- Cannot deal with high dimensional inputs (larger search space).
            -- Cannot correctly recovering the original Trojan shape. 
                -- (l1 norm dosenot performs well in high dimensional space). 
            -- Including false positive.
                -- (dosenot filtering out adversarial samples).
            -- Cannot obtaining high fidelity Trojan. 
                -- (dosenot adding any constraints on delta). 
                
    3.2 Problem scope. (goes to 2.2)
        -- Extracting a high fidelity backdoor from a trained model with clean testing data. 
        -- Mainly focusing on injecting one Trojan into only one label of a model.
        -- Trojan with regular shape (square and circle).
        -- Added at the corner of an input sample.

4. Proposed Technique. (2 - 3 pages) (weekend)
    4.1 Design principles.
        -- Sharking searching space.
            -- Using other norm instead of l1 (nuclear and elastic-net).
        -- Filtering out false positive.
            -- Adding smoothness loss.
        -- Obtaining a high fidelity Trojan. 
            -- Adding similar loss on delta.
            -- integrating the explanation part.
    4.2 Technical details.
        4.1 Each term in the loss function.
            -- Attack loss.
            -- Trojan loss (Explanation).
            -- Remain loss.
            -- Mask loss.
                -- sparsity. 
                -- smoothness.
            -- Delta loss. 
                -- sparsity. 
                -- smoothness.
        4.2 Training strategy.
        4.3 Metric for Identifying Trojan.
            $log(l_0||mask||/(n*n)) - log(Attack_Accuracy)$
            -- Model with one Trojan:
                -- minimum value.
            -- Model with multiple Trojans:
                -- Outlier detection.
        4.4 Hyper-parameter decay.
        4.5 Discussion
            Why not directly performing the sp approach on the low D representation.

5. Evaluation. (3-4 pages)
    5.1 Experimental Setup.
    Datasets and attacks:
        BadNet-gtsrb: (32*32*3) (Progress: Done)
        BadNet-ImageNet: (224*224*3) (Progress: Done.)
        Trojan Attack (NDSS https://github.com/PurduePAML/TrojanNN): VGG Face (224*224*3) (Progress: Done) 
        TODO: Imagenet: resnet; 2 in 1; 2 in 2;
        
    Model architectures and Accuracy:
        
    5.2 Experimental Design.
        Main Experiment: One Infected label with one Trojan.
        Factors:
            Shape: 1. Square with single color (black or white, depends on the background of the dataset).
                   2. Circle with more complex color: Firefox logo (2).
            Location: Diagonal location (Upper left and lower right or Upper right and lower left) (2).
            Size: Four different size level (5).
    
    5.3 Experimental Results.
        -- Detected or not.
        -- Fidelity.
            -- mask l1 distance.
            -- Trojan l2 distance.

    5.4 Other Experiments (Using one dataset and selecting one setting to run the experiment).
        -- Multiple Infected Labels with Separate Triggers.
            -- MAD detection.
        -- Single Infected Label with Multiple Triggers
            -- MAD detection.
        -- Water-mark backdoor and Source-label-specific (Partial) Backdoor. 
    5.5 Sensitivity to the parameters.
    
    (model complexity vs. detection effectiveness)

6. Discussion and Future Works (0.5)
    Limitations ...
    Future direction (learning-to-optimize ...)
    
7. Conclusion (1/4)

3. Related Works (1 page)
        2.2.1 trigger detection.
        2.2.2 Trojan detection.
        2.3.3 Trojan elimination.
        
Note: This outline dose not include detecting Trojan at low D space and then come back. Leave this a future work if we can get good results on the original inputs.

==> table/dataset.tex <==
% \begin{table*}[hbtp]
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% % \multirow{2}{*}{} & \multicolumn{2}{c|}{GTSRB}       & \multicolumn{2}{c|}{ImageNet}    & \multicolumn{2}{c|}{PubFig}      \\ \cline{2-7} 
% Task & Dataset & Network & Image Size & \#Classes & \#Training Samples & Attack Type \\ \hline
% Traffic Sign Recognition & GTSRB & 6 Conv + 2 MaxPooling & (32, 32, 3) & 43 & 35288 & BadNet \cite{gu2017badnets} \\ \hline
% Visual Object Recognition & ImageNet & VGG16 \cite{simonyan2014very} & (224, 224, 3) & 50 & 20,000 & BadNet \cite{gu2017badnets} \\ \hline
% Face Recognition & LFW & VGG16 \cite{simonyan2014very} & (224, 224, 3) & 2622 & 2,622 & Trojan Attack \cite{Trojannn} \\ \hline
% \end{tabular}
% \caption{Details about the selected Datasets. Note that we use a 50-class subset of ImageNet in our evaluation for computational efficiency.}
% \label{tab:datasets}
% \end{table*}

\begin{table*}[hbtp]
\begin{tabular}{|c|c|c|c|c|c|}
\hline
% \multirow{2}{*}{} & \multicolumn{2}{c|}{GTSRB}       & \multicolumn{2}{c|}{ImageNet}    & \multicolumn{2}{c|}{PubFig}      \\ \cline{2-7} 
Task & Dataset & Image Size & \#Classes & \#Training Samples & Attack Type \\ \hline
Traffic Sign Recognition & GTSRB  & (32, 32, 3) & 43 & 35288 & BadNet \cite{gu2017badnets} \\ \hline
Visual Object Recognition & ImageNet  & (224, 224, 3) & 50 & 20,000 & BadNet \cite{gu2017badnets} \\ \hline
Face Recognition & LFW  & (224, 224, 3) & 2622 & 2,622 & Trojan Attack \cite{Trojannn} \\ \hline
\end{tabular}
\caption{The selected Datasets. Note that we use a 50-class subset of ImageNet in our evaluation for computational efficiency.}
\label{tab:datasets}
\end{table*}

==> table/hyper_used.tex <==
\begin{table}[hbtp]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    Hyper-parameters & GTSRB & ImageNet \& LFW \\
    \hline
    \#Epochs & 500 & 500 \\
    \hline
    Learning Rate & $1\times e^{-3}$ & $1\times e^{-3}$ \\
    \hline
    Optimizor & {\tt Adam} & {\tt Adam}\\
    \hline
    Mask Regularizor & elastic net & elastic net \\
    \hline
    Delta Regularizor & elasetic net & $l_1$ \\
    \hline
    $\lambda_1$ & $1\times e^{-6}$ & $1\times e^{-3}$ \\
    \hline
    $\lambda_2$ & $1\times e^{-5}$ & $1\times e^{-5}$\\
    \hline
    $\lambda_3$ & $1\times e^{-7}$ & $1\times e^{-6}$ \\
    \hline
    $\lambda_4$ & $1\times e^{-8}$ & $1\times e^{-9}$ \\
    \hline
    $\lambda_5$ & $1\times e^{-6}$ & $1\times e^{-6}$ \\
    \hline
    $\lambda_6$ & $1\times e^{-2}$ & $1\times e^{-2}$ \\
    \hline
    \end{tabular}
    \caption{The values of the hyper-parameters used in our experiments.}
    \label{tab:hyper_used}
    \vspace{-5pt}
\end{table}

==> table/trojans.tex <==
\begin{table}[hbtp]
    \centering
    \begin{tabular}{|c|c|}
    \hline
    Attack Method & Trojan Shape \\
    \hline
    BadNet \cite{gu2017badnets} & \includegraphics[width=0.1\textwidth]{img/GTSRB/square/br_60.png} \\
    \hline
    Trojan Attack \cite{Trojannn} & \includegraphics[width=0.1\textwidth]{img/trojans/trojan.jpg} \\
    \hline
    \end{tabular}
    \caption{Trojan added by Different Attacks}
    \label{tab:trojans}
\end{table}
